Understanding video streaming algorithms in the wild

While video streaming algorithms are a hot research area, with interesting new approaches proposed every few months, little is known about the behavior of the streaming algorithms deployed across large online streaming platforms that account for a substantial fraction of Internet traffic. We thus study adaptive bitrate streaming algorithms in use at 10 such video platforms with diverse target audiences. We collect traces of each video player's response to controlled variations in network bandwidth, and examine the algorithmic behavior: how risk averse is an algorithm in terms of target buffer; how long does it takes to reach a stable state after startup; how reactive is it in attempting to match bandwidth versus operating stably; how efficiently does it use the available network bandwidth; etc. We find that deployed algorithms exhibit a wide spectrum of behaviors across these axes, indicating the lack of a consensus one-size-fits-all solution. We also find evidence that most deployed algorithms are tuned towards stable behavior rather than fast adaptation to bandwidth variations, some are tuned towards a visual perception metric rather than a bitrate-based metric, and many leave a surprisingly large amount of the available bandwidth unused.

==> TODO.tex <==
- Check the citations for obvious errors or missing details 

######### Changes Proposed (Max)
I in general do not know how much additional work we want (have) to put into making the paper "prettier". 
#### General Things
    - Annotate the things the reviewers have mentioned within the text and add explanations where we feel that it the overall text does not answer the question to the full extent. (Medium Priority)
    - I can generate a "cleanish" version of the sampling script to put in a public repo. (Medium Priority)
#### As proposed by reviewers (specific changes)
    - Add Paragraph how we collect the metadata (High Priority)
        -> This is actually a hacking process which is different for every provider but we can definitely release a script for every provider which we tested with which can (in the current version of the player) download AND generate the necessary metadata. 
    - Look at the behaviour when rebuffering (#28C) (Low Priority)
        -> We would have to replace another analysis with that one. I don't know if that is a good idea as the paper might loose some of its well "roundedness" through replacing another analysis.
    - Some reviewers had a problem with the analysis of the proxy impact. We might have to consider going more into depth here. (High Priority)
        -> Why ZDF and YouTube show a divergence in mean QoE is not currently clear to me and this would need some more investigation. 
#### Timeline
I have to prepare for the submission at the 15th for ATC. I certainly can skim some time off my schedule for polishing the the submission. I though also have to do the same for my poster. After the hand in we'll be a bit pressed for time as the better half of the week after that one will be taken up by the retreat. What are your thoughts ? 

==> tables_evaluation/general_stats_table.tex <==
\begin{table*}
\centering
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{llllll}
         Provider & $ \frac{Rebuffer}{Played} $ & $ \frac{\# Rebuffer}{Played} $ & $ \overline{\frac{Switches}{s}}$ & $ \overline{Mbps} $ & $ \overline{VMAF} $ \\
\hline
    \textbf{Arte} &             $0.273 \pm 0.3$ &               $0.028 \pm 0.03$ &                 $0.015 \pm 0.02$ &    $1.021 \pm 0.68$ &  $30.356 \pm 31.99$ \\
  \textbf{Fandom} &            $0.008 \pm 0.02$ &                $0.003 \pm 0.0$ &                 $0.021 \pm 0.02$ &    $1.263 \pm 1.07$ &  $60.495 \pm 30.75$ \\
 \textbf{Pornhub} &            $0.008 \pm 0.02$ &                $0.003 \pm 0.0$ &                 $0.013 \pm 0.01$ &    $1.234 \pm 0.76$ &  $74.095 \pm 19.55$ \\
     \textbf{SRF} &            $0.033 \pm 0.13$ &               $0.005 \pm 0.01$ &                  $0.02 \pm 0.02$ &    $1.356 \pm 1.07$ &  $61.064 \pm 30.48$ \\
  \textbf{TubiTV} &            $0.161 \pm 0.69$ &               $0.018 \pm 0.04$ &                 $0.009 \pm 0.01$ &     $1.188 \pm 0.7$ &  $51.994 \pm 26.17$ \\
  \textbf{Twitch} &            $0.237 \pm 0.53$ &               $0.011 \pm 0.02$ &                 $0.015 \pm 0.01$ &    $1.231 \pm 0.84$ &    $42.0 \pm 21.46$ \\
   \textbf{Vimeo} &            $0.083 \pm 0.21$ &               $0.011 \pm 0.02$ &                 $0.009 \pm 0.01$ &    $1.238 \pm 1.47$ &  $57.198 \pm 29.66$ \\
 \textbf{XVideos} &            $0.183 \pm 1.51$ &               $0.003 \pm 0.01$ &                 $0.009 \pm 0.01$ &    $0.815 \pm 0.72$ &  $47.323 \pm 33.95$ \\
 \textbf{YouTube} &            $0.126 \pm 0.23$ &               $0.009 \pm 0.01$ &                 $0.009 \pm 0.01$ &    $1.522 \pm 0.85$ &  $70.041 \pm 22.32$ \\
     \textbf{ZDF} &            $0.051 \pm 0.13$ &               $0.004 \pm 0.01$ &                 $0.023 \pm 0.01$ &    $1.671 \pm 1.01$ &   $79.69 \pm 19.42$ \\
\hline
\end{tabular}
\vspace{8pt}
\caption{}
\vspace{-0.1in}
\end{table*}
